Optimal Control of Material Micro-Structures

In this paper, we consider the optimal control of material micro-structures. Such material micro-structures are modeled by the so-called phase field model. We study the underlying physical structure of the model and propose a data based approach for its optimal control, along with a comparison to the control using a state of the art Reinforcement Learning (RL) algorithm. Simulation results show the feasibility of optimally controlling such micro-structures to attain desired material properties and complex target micro-structures.

==> D2C-2.tex <==
\section{Decoupled Data based Control (D2C)}
\label{sec4}
This section presents our decoupled data-based control (D2C) algorithm. We outline the open loop and closed loop design components of D2C below.
%
\subsection{Open-Loop Trajectory Design}
\label{open_loop_traj_design}
%An open-loop trajectory is designed by solving the corresponding problem in subsection \ref{OL_CL_problems}. However, since we are solving it in a model-free manner, we need a suitable formulation that can efficiently compute the solution.
We present an ILQR \cite{ilqg2} based method to solve the open-loop optimization problem. ILQR typically requires the availability of analytical system Jacobian, and thus, cannot be directly applied when such analytical gradient information is unavailable (much like Nonlinear Programming software whose efficiency depends on availability of analytical gradients and Hessians).  In order to make it an (analytical) model-free algorithm, it is sufficient to obtain estimates of the system Jacobians from simulations, and a sample-efficient randomized way of doing so is described in the following subsection. Since ILQR is a well-established framework, we skip the details and instead present a psuedocode in algorithm \ref{model_free_DDP_OL}. \textit{Please refer to the supplementary document to see why the ILQR scheme is particularly attractive and can be guaranteed to converge to a global minimum for the open loop problem even though the problem is non-convex. We also note that any (analytical) model-free open loop design technique can be swapped for ILQR in this step.}
\subsubsection{Estimation of Jacobians: Linear Least Squares by Central Difference (LLS-CD)}
\label{sys_id_solve}
% We make a preliminary analysis on the number of evaluations required in the above algorithm. If the horizon is `$h$' and the number of iterations required to converge are `$n$', the algorithm requires us to estimate each of the $f_{\bf x_t}$ and $f_{\bf u_t}$ `$nh$' times. 


% \begin{equation*}
% \begin{split}
%     &f({\bf \bar{x}_t} + \delta {\bf x_t}, {\bf \bar{u}_t} + \delta {\bf u_t}) = f({\bf \bar{x}_t}, {\bf \bar{u}_t}) + \begin{bmatrix} f_{\bf x_t}  f_{\bf u_t} \end{bmatrix} \begin{bmatrix}  \delta {\bf x_t} \\ \delta {\bf u_t} \end{bmatrix} + \\&\frac{1}{2} \begin{bmatrix} \delta {\bf x_t}^T  \delta {\bf u_t}^T \end{bmatrix} \begin{bmatrix} f_{\bf x_t x_t}  f_{\bf x_t u_t}\\ f_{\bf u_t x_t}  f_{\bf u_t u_t}\end{bmatrix} \begin{bmatrix} \delta {\bf x_t} \\ \delta {\bf u_t}\end{bmatrix} +
%     O(\| \delta {\bf x_t}\|^3 + \| \delta {\bf u_t}\|^3)\\
%     &f({\bf \bar{x}_t} - \delta {\bf x_t}, {\bf \bar{u}_t} - \delta {\bf u_t}) = f({\bf \bar{x}_t}, {\bf \bar{u}_t}) - \begin{bmatrix} f_{\bf x_t} f_{\bf u_t} \end{bmatrix} \begin{bmatrix}  \delta {\bf x_t} \\ \delta {\bf u_t} \end{bmatrix} + \\&\frac{1}{2} \begin{bmatrix} \delta {\bf x_t}^T \delta {\bf u_t}^T \end{bmatrix} \begin{bmatrix} f_{\bf x_t x_t}  f_{\bf x_t u_t}\\ f_{\bf u_t x_t}  f_{\bf u_t u_t}\end{bmatrix} \begin{bmatrix} \delta {\bf x_t} \\ \delta {\bf u_t}\end{bmatrix}+
%     O(\| \delta {\bf x_t}\|^3 + \| \delta {\bf u_t}\|^3)\\
%   \end{split}
% \end{equation*}
From the Taylor's expansions of `\textit{h}' (for generality, \textit{h} is the non-linear model of Section 2)  about the nominal trajectory $({\bar{x}_t}, \bar{u}_t)$ on both the positive and the negative sides, we obtain the following central difference equation:\\
$
    h(\bar{x}_t+ \delta  x_t, \bar{u}_t + \delta u_t) - h(\bar{x}_t - \delta  x_t, \bar{u}_t - \delta u_t) =~2 \begin{bmatrix} h_{x_t} & h_{u_t} \end{bmatrix} \begin{bmatrix}  \delta  x_t \\ \delta u_t \end{bmatrix} + O(\| \delta  x_t\|^2 + \| \delta u_t\|^2).
$

%Multiplying by $\begin{bmatrix} \delta {\bf x_t}^T & \delta {\bf u_t}^T \end{bmatrix}$ on both sides, the above equation can be written as,
\begin{comment}
\begin{equation*}
    \begin{split}
    \begin{bmatrix}h({\bf \bar{x}_t} + \delta {\bf x_t}, {\bf \bar{u}_t} + \delta {\bf u_t}) - h({\bf \bar{x}_t} - \delta {\bf x_t}, {\bf \bar{u}_t} - \delta {\bf u_t})\end{bmatrix} \times \begin{bmatrix} \delta {\bf x_t}^T & \delta {\bf u_t}^T \end{bmatrix} 
    % &= 2 \begin{bmatrix} f_{\bf x_t} & f_{\bf u_t} \end{bmatrix} \begin{bmatrix}  \delta {\bf x_t} \\ \delta {\bf u_t} \end{bmatrix} \begin{bmatrix} \delta {\bf x_t}^T & \delta {\bf u_t}^T \end{bmatrix}+ O(\| \delta {\bf x_t}\|^4 + \| \delta {\bf u_t}\|^4)\\
     \\
     =2 \begin{bmatrix} h_{\bf x_t} & h_{\bf u_t} \end{bmatrix} \begin{bmatrix}  \delta {\bf x_t} \delta {\bf x_t}^T & \delta {\bf x_t} \delta {\bf u_t}^T \\ \delta {\bf u_t} \delta {\bf x_t}^T  & \delta {\bf u_t} \delta {\bf u_t}^T \end{bmatrix}+ O(\| \delta {\bf x_t}\|^4 + \| \delta {\bf u_t}\|^4)
     \end{split}
\end{equation*}
\end{comment}
% \begin{equation*}
%     \begin{split}
%     &\begin{bmatrix}f({\bf \bar{x}_t} + \delta {\bf x_t}, {\bf \bar{u}_t} + \delta {\bf u_t}) - f({\bf \bar{x}_t} - \delta {\bf x_t}, {\bf \bar{u}_t} - \delta {\bf u_t})\end{bmatrix} \times\\
%     &\begin{bmatrix} \delta {\bf x_t}^T & \delta {\bf u_t}^T \end{bmatrix} \begin{bmatrix}  \delta {\bf x_t} \delta {\bf x_t}^T & \delta {\bf x_t} \delta {\bf u_t}^T \\ \delta {\bf u_t} \delta {\bf x_t}^T  & \delta {\bf u_t} \delta {\bf u_t}^T \end{bmatrix}^{-1} = \\&2 \begin{bmatrix} f_{\bf x_t} & f_{\bf u_t} \end{bmatrix} +
%      O(\| \delta {\bf x_t}\|^2 + \| \delta {\bf u_t}\|^2)
%      \end{split}
% \end{equation*}
% $\implies$ 
%\begin{equation}
 %   \begin{split}
  %  \begin{bmatrix} f_{\bf x_t} & f_{\bf u_t} \end{bmatrix} =~&\frac{1}{2}\begin{bmatrix} f({\bf \bar{x}_t} + \delta {\bf x_t}, {\bf \bar{u}_t} + \delta {\bf u_t}) - f({\bf \bar{x}_t} - \delta {\bf x_t}, {\bf \bar{u}_t} - \delta {\bf u_t})\end{bmatrix} \times\\&\begin{bmatrix} \delta {\bf x_t}^T & \delta {\bf u_t}^T \end{bmatrix} \begin{bmatrix}  \delta {\bf x_t} \delta {\bf x_t}^T & \delta {\bf x_t} \delta {\bf u_t}^T \\ \delta {\bf u_t} \delta {\bf x_t}^T  & \delta {\bf u_t} \delta {\bf u_t}^T \end{bmatrix}^{-1} + O(\| \delta {\bf x_t}\|^2 + \| \delta {\bf u_t}\|^2)
   %  \label{eq : model_free_DDP_jacobian_raw}
    % \end{split}
%\end{equation}
The above equation can now be used to estimate the Jacobians, $h_{x_t}$ and $h_{u_t}$ by sampling $\delta x_t$ and $\delta u_t$. %It is noted that the above formulation requires only 2 evaluations of $f(.)$, given the nominal state and control $\-$ (${\bf \bar{x}_t},{\bf \bar{u}_t}$). The remaining terms (also, the error in the evaluation) are of the order that is quadratic in $\delta {\bf x_t}$ and $\delta {\bf u_t}$.\\ %The following extends equation \eqref{eq : model_free_DDP_jacobian_raw} to be used in a practical implementations (sampling).\\
We choose the distribution of $\delta x_t$ and $\delta u_t$ to be i.i.d. Gaussian distributed random variables with zero mean and a standard deviation of $\sigma$.
 Denote the random samples as $\delta {X_t} = \begin{bmatrix} \delta {x_t^1}& \delta {x_t^2}& \ldots &\delta {x_t^{n_s}}\end{bmatrix}$, $\delta {U_t} = \begin{bmatrix} \delta {u_t^1} &\delta {u_t^2}& \ldots& \delta {u_t^{n_s}}\end{bmatrix}$, and $\delta {Y_t} = [\delta {X_t} \, \delta {U_t}]$. Then $\begin{bmatrix} h_{x_t} & h_{u_t} \end{bmatrix}$ is given by the following (via standard least squares) :
\begin{equation}
    %\begin{split}
    \begin{bmatrix} h_{x_t} & h_{u_t} \end{bmatrix} =\begin{bmatrix} h({\bar{x}_t} + \delta {x_t^1}, {\bar{u}_t} + \delta {u_t^1}) - h({\bar{x}_t} - \delta {x_t^1}, {\bar{u}_t} - \delta {u_t^1})\\ h({\bar{x}_t} + \delta {x_t^2}, {\bar{u}_t} + \delta {u_t^2}) - h({\bar{x}_t} - \delta {x_t^2}, {\bar{u}_t} - \delta {u_t^2}) \\ \vdots  \\h({\bar{x}_t} + \delta {x_t^{n_s}}, {\bar{u}_t} + \delta {u_t^{n_s}}) - h({\bar{x}_t} - \delta {x_t^{n_s}}, {\bar{u}_t} - \delta {u_t^{n_s}})\end{bmatrix} \delta {Y_t^{T}}({\delta {Y_t}\delta {Y_t^T}})^{-1},
     \label{eq : model_free_DDP_jacobian}
     %\end{split}
\end{equation}
where, 
$
(\delta {Y_t}\delta {Y_t^T})
\approx \sigma^2 (n_s - 1){\text I}_{(n_x+n_u) \times (n_x+n_u)}
$ if $n_s$ is sufficiently large
(see the supplementary material for a detailed version of the derivation).\\
\textit{Sample Complexity.} Given that we have a sufficient number of samples `$n_s$' (typically `$O(n_x + n_u)$' are sufficient), the above approximation holds good. Compare this with the $O(n_x(n_x+n_u))$ samples required by finite differencing schemes \cite{ILQG_complex_behaviors}. Please see the supplementary document to understand the analytical reason behind the sample efficiency of such randomized sampling and the empirical results to see the practical benefit over FD.
% Since the inversion of an identity matrix is trivial and always exists, the above matrix is invertible in equation \eqref{eq : model_free_DDP_jacobian}. 
Henceforth, we will refer to this method as `Linear Least Squares by Central Difference (LLS-CD)'. The entire algorithm is summarized together in Algorithm \ref{model_free_DDP_OL}. The detailed forward and backward pass functions are shown in Algorithm 2 and 3 respectively in the supplementary material.
\begin{algorithm}[!htbp]
\footnotesize
  \caption{\strut Open-loop trajectory optimization via model-free ILQR}
  {\bf Input:} Initial State - ${\bf x_0}$, System parameters - $\mathcal{P}$\;
  $k \gets 1$. ~~\CommentSty{/* Initialize the iteration number $k$ to 1.*/}\\
  $forward\_pass\_flag$ = true. \\
  \CommentSty{/* Run until the difference in costs between subsequent iterations is less an $\epsilon$ fraction of the former cost.*/}\\
  \While {$k==1$ {\textnormal{or}} $({\text cost}(\mathbb{T}_{nom}^{k})/{\text cost}(\mathbb{T}_{nom}^{k-1})) < 1 + \epsilon$}{
  \CommentSty{/*Each iteration has a backward pass followed by a forward pass.*/}\\
  \{$k^{k}_{0:N-1}, K^{k}_{0:N-1}$\}, $backward\_pass\_success\_flag$ $=$ Backward Pass($\mathbb{T}_{nom}^{k}$, $\mathcal{P}$).\\
  \If{backward\_pass\_success\_flag == true}{
      $\mathbb{T}_{nom}^{k+1}, forward\_pass\_flag$ $=$ Forward Pass($\mathbb{T}_{nom}^{k}$,$\{k^{k}_{0:N-1}, K^k_{0:N-1}\}$, $\mathcal{P}$).\\
      \While{forward\_pass\_flag == false}{
            $\mathbb{T}_{nom}^{k+1}, forward\_pass\_flag$ $=$ Forward Pass($\mathbb{T}_{nom}^{k}$,$\{k^{k}_{0:N-1}, K^k_{0:N-1}\}$, $\mathcal{P}$).\\
            Reduce $\alpha$ from $\mathcal{P}$.    
        }
      }
   \Else{
        Increase $\mu$ from $\mathcal{P}$.~~\CommentSty{/* Regularization step */}\\
    }
      $k \leftarrow k + 1$. \\
  $\mathbb{T}^{*}_{nom} \gets \mathbb{T}^{k+1}_{nom}$.\\
  }
  
  {\bf return $\mathbb{T}^{*}_{nom}$}\\
  \label{model_free_DDP_OL}
\end{algorithm}
\subsection{Closed Loop Design}
\label{lqr_design}
As discussed in the previous section, a time-varying LQR feedback law is used as a surrogate for the minimum variance problem. The LQR gains $\{K_{1:N-1}\}$ can be fully determined if $Q_t$, $R_t$, $A_t$ and $B_t$ are known. The first two are the tuning parameters in the cost function. Determining $A_t (\equiv h_{x_t})$ and $B_t (\equiv h_{u_t})$ for a linear system is a system identification problem that can be solved by `LLS-CD' as described above \ref{sys_id_solve}. 

==> DDPGAlgorithm.tex <==
\subsection{\textbf{DDPG Algorithm}}
\label{sec:ddpg}
Deep Deterministic Policy Gradient (DDPG) is a policy-gradient based off-policy reinforcement learning algorithm that operates in continuous state and action spaces. It relies on two function approximation networks one each for the actor and the critic. The critic network estimates the $Q(s, a)$ value given the state and the action taken, while the actor network engenders a policy given the current state. Neural networks are employed to represent the networks. 

The off-policy characteristic of the algorithm employs a separate behavioral policy by introducing additive noise to the policy output obtained from the actor network. The critic network minimizes loss based on the temporal-difference (TD) error and the actor network uses the deterministic policy gradient theorem to update its policy gradient as shown below:

Critic update by minimizing the loss: 
\begin{equation*}
    L = \frac{1}{N} \Sigma_{i}(y_i - Q(s_i, a_i| \theta^{Q}))^2
\end{equation*}

Actor policy gradient update:
\begin{equation*}
    \nabla_{\theta^{\mu}} \approx \frac{1}{N} \Sigma_i \nabla_a Q(s,a|\theta^{Q})|_{s=s_i,a=\mu(s_i)} \nabla_{\theta^{\mu}} \mu(s|\theta^{\mu})|_{s_i}
\end{equation*}

The actor and the critic networks consist of two hidden layers with the first layer containing 400 ('{\it relu}' activated) units followed by the second layer containing 300 ('{\it relu}' activated) units. The output layer of the actor network has the number of ('tanh' activated) units equal to that of the number of actions in the action space.  

Target networks one each for the actor and the critic are employed for a gradual update of network parameters, thereby reducing the oscillations and a better training stability. The target networks are updated at $\tau = 0.001$. Experience replay is another technique that improves the stability of training by training the network with a batch of randomized data samples from its experience. We have used a batch size of 32 for the inverted pendulum and the cart pole examples, whereas it is 64 for the rest. Finally, the networks are compiled using Adams' optimizer with a learning rate of 0.001. 

To account for state-space exploration, the behavioral policy consists of an off-policy term arising from a random process. We obtain discrete samples from the Ornstein-Uhlenbeck (OU) process to generate noise as followed in the original DDPG method. The OU process has mean-reverting property and produces temporally correlated noise samples as follows:
\begin{equation*}
    dx_t = \Theta (\mu - x_t)dt + \sigma dW
\end{equation*}
where $\Theta$ indicates how fast the process reverts to mean, $\mu$ is the equilibrium or the mean value and $\sigma$ corresponds to the degree of volatility of the process. $\Theta$ is set to 0.15, $\mu$ to 0 and $\sigma$ is annealed from 0.35 to 0.05 over the training process. 

==> FAQ <==
***********************************************************************
Question 1:
Could  you please send the information regarding importing 
encapsulated postscript (*.eps) files (figures)  
into your *.tex and *.sty (asme.tex or asme.sty) provided. 
What should be the command I should add to the file and in which file, 
in *.sty or *.tex. Usually I add \input epsf in my *.tex file. 
Please let me know this way of importing the figure is acceptable.

Answer:
You may use the 'epsfig' package to incorporate an encapsulated postscript
figure into your document.  To include the package in LaTeX2e, use
"\usepackage{epsfig}" in the preamble of your document.  Use
"\epsfig{file=file.eps}" to incorporate the eps file in the figure environment.  
You may use width and/or height arguments to change the size
of the original figure, e.g. "\epsfig{file=file.eps,width=3in}."

If you are using LaTeX 2.09, use "\input{psfig}" in the preamble and use
"\psfig{figure=file.eps}" to include the eps file.  The height and width
arguments are the same.

Note: the argument for \epsfig{} and \psfig{} starts with 
"file=" and "figure=", respectively.

***********************************************************************
Question 2:
I am current preparing a paper to be submitted in an ASME conference.
There is a problem we are not able to solve. The problem is the
display of lower case Greek bold face font. 
Normally, the command 
\mbox{\boldmath${  ....  }$\unboldmath}
will do it. However, using the ASME template, this command seem not
function. I wonder if you had come across this problem before and
would share you experience with us.

Answer:
In LaTeX2e, use the \mathbf{} command
to make a bold math character.  
If that doesn't work, you will have to use an ams-LaTeX package.  

***********************************************************************
Question 3: 
How can I get bold italics?

Answer:
try \newcommand{\bAC}{\mbox{$\mathbf{AC}$}}
You could also try \textbf{\emph AC}

***********************************************************************
Question 4: 

I've been using your LaTeX2e asme2e.cls package to prepare a paper
for an upcoming conference, but have been having some trouble with the
fonts.  I was wondering if I might be able to ask you for a bit of
advice.

It seems as if none of the headings, titles, etc, are showing
up bold as they are supposed to.  When I run LaTeX, I get the
following...

{co.eng.caltech.edu:7} latex paper.tex
This is TeX, Version 3.1415 (C version 6.1)
(paper.tex
LaTeX2e <1994/12/01> patch level 1
(asme2e.cls
Document Class: asme2e 1997/04/10 v1.0 Standard LaTeX document class
(/ccovol/tex3/tex/latex/base/ifthen.sty)
(/ccovol/tex3/tex/latex/packages/psnfss/times.sty)
(/ccovol/tex3/tex/latex/packages/psnfss/mathptm.sty)
(/ccovol/tex3/tex/latex/packages/psnfss/pifont.sty
No file Upzd.fd.

LaTeX Font Warning: Font shape `U/pzd/m/n ' undefined
(Font)              using `U/cmr/m/n' instead on input line 57.

No file Upsy.fd.

LaTeX Font Warning: Font shape `U/psy/m/n ' undefined
(Font)              using `U/cmr/m/n' instead on input line 58.




...and so on.

I noticed in the README2 file that there were some issues pertaining
to fonts.  Apparently I need to make sure that a new font package
(PSNFSS) is installed.  Does LaTeX's call to 

(/ccovol/tex3/tex/latex/packages/psnfss/times.sty)

imply that the sysadmins here have already done this?  In any case, I
tried to find the font packages at

http://tug2.cs.umb.edu/ctan/tex-archive/macros/latex/packages/psnfss/

but that address appears to have expired.  

If it is just a matter of installing these fonts, do you know of a new
address where I can get them?  And if it doesn't seem to be just a
problem of installing these fonts, do you have any ideas as to what
might be wrong?


Answer:
The problem is the  "pifont.sty" package uses the "Upzd.fd" and the "Upsy.fd"
font description files, which are missing in your installation of psnfss.  A
quick fix is to download the missing files from CTAN.  Point your browser to
http://www.ctan.org and click on the search link to search for the two files.
Download them to the same directory as your paper and rerun LaTeX2e.
You should ask your system administrators to install psnfss with the proper font
description files.



***********************************************************************
Question 5: 

How do you use .jgp and .png images as figures in LaTex when using PDF Texify?

Answer by Adam Pautsch at agpautsch@wisc.edu:
To include images, you must load the package "graphicx" in the preamble of 
the document. With the image file in the same folder as the .tex file, use 
the line "\includegraphics[keepaspectratio,width=3in]{filename.jgp}" to 
insert the image file. This may be included inside of a "figure" environment, 
which will allow for automatic captioning with the "\caption{}" command.

The images included in this manner will only appear when the "draft" option is
not used. When "draft" is used as an option, a box represnting an image with
the image's filename will appear in its place.

More information about handling images of different formats may be found at
     http://www.tex.ac.uk/cgi-bin/texfaq2html?label=dvipsgraphics
     http://www.tex.ac.uk/cgi-bin/texfaq2html?label=pdftexgraphics



==> Hybrid.tex <==
\subsubsection{Warm Starting(Model Based Approach)}
In  this  section, we derive a simple control scheme to control the inputs to each grid point in the material, so as to reach the desired phase distribution. In order to achieve this, we exploit the Allen-Cahn dynamics along with the assumptions of a periodic boundary condition to get a better initial estimate for the control scheme.

The Allen-Cahn equation has an interesting structure. Suppose we assume our system to be a single cell/pixel i.e. discretized as a 1X1 matrix. Owing to our assumption of a periodic boundary condition, the diffusion term effectively vanishes, i.e. $\nabla^2 \phi=0$. Thus, our dynamics reduce to 
\begin{equation}
    \frac{\partial \phi}{\partial t}=-M\frac{\partial f}{\partial \phi}=-M(4\phi^3+2T\phi+h)
\end{equation}
Thus, the simplified model reduces to a temporal differential equation instead of a complex spatio-temporal partial differential equation. This single pixel system is then fed to our iLQR-based control scheme, to generate a look-up table (of sorts) for a control trajectory from the given initial state $\phi_0$ to both stable final states $\phi_f=\pm 1$. 

The control trajectories thus obtained are mapped to any desired final state structure, and serve as an improved initial guess for the main algorithm, i.e. now the algorithm only has to optimize for the diffusion term.


\begin{figure}[!htb]
%\captionsetup{width=1\linewidth}



\begin{multicols}{2}
    %\hspace{3.2cm}
      \subfloat[]{\includegraphics[width=1\linewidth]{images/Hybrid/episodic_cost_training_original.png}}    
      \subfloat[]{\includegraphics[width=\linewidth]{images/Hybrid/episodic_cost_training_hyb.png}}
      %\subfloat[t=1.25s]{\includegraphics[width=0.8\linewidth]{images/50per/file49.png}}\\
      
         
\end{multicols}
%\begin{multicols}{6}
%\captionsetup{width=.75\textwidth}
    \caption{{Open loop training with starting guess initialised as (a)random control trajectory with zero mean, 
    (b)model based approach}} 
%\end{multicols}

\label{hyb_train}
\end{figure}

\begin{figure}
    %\centering
    \includegraphics[width=\linewidth]{images/Hybrid/trajComp.png}
    \caption{Comparing trajectories from model-based single-pixel method(no diffusion) with the optimized trajectory(with diffusion)}
    \label{fig:MSE_hyb}
\end{figure}



==> ILQR.tex <==
\subsection{Iterative Linear Quadratic Regulator Details}

% The Iterative LQR algorithm implemented here is a variation of the classical Differential Dynamic Programming(DDP) algorithm, wherein we constrain ourselves to just the first derivative of the dynamics.
% Let $U_t=\{u_i\}_{i=t}^{T-1}$. The cost-to-go is, thus, defined as
% \begin{equation*}
%     J_t(x,U_t)=\sum_{i=t}^{T-1} c(x_t, u_t)+\phi(x_T)
% \end{equation*}

% The value function at time \textit{t} is the cost-to-go given the minimising control sequence,
% \begin{equation*}
%     V_t(x) \equiv \min_{U_t} J_t(x, U_t).
% \end{equation*}

% Setting $V_T(x)=\phi(x_T)$, we can apply the Dynamic Programming Principle, which reduces the minimization over a sequence of controls to a sequence of minimizations over a single
% control, proceeding backwards in time:
% \begin{align*}
%     V_t(x)=\min_{u_t} [c(x_t,u_t)+V_{t+1}(f(x_t,u_t))], \\
%     Q_t(x)=arg\min_{u_t} [c(x_t,u_t)+V_{t+1}(f(x_t,u_t))]
% \end{align*}
% We define the action-value function as a function of perturbations around the pair $(x_t, u_t)$:
% \begin{align*}
%     Q_t(\delta x_t, \delta u_t)=c(x_t+\delta x_t, u_t+\delta u_t)-c(x_t, u_t) +\\
%     V_{t+1}(f(x_t+\delta x_t, u_t+\delta u_t))-V_{t+1}(f(x_t, u_t))
% \end{align*}
% and expand to the second order
% \begin{align}
%     Q_t(\delta x_t, \delta u_t) \approx \frac{1}{2}\begin{bmatrix}
%     1\\
%     \delta x_t\\
%     \delta u_t
%     \end{bmatrix}^T \begin{bmatrix}
%     0 &Q_x^T &Q_u^T\\
%     Q_x &Q_{xx} &Q_{xu}\\
%     Q_u &Q_{ux} &Q_{uu}
%     \end{bmatrix} \begin{bmatrix}
%     1\\
%     \delta x_t\\
%     \delta u_t
%     \end{bmatrix}
% \label{eq:ilqg_2nd_order}
% \end{align}
% The expansion coefficients can be written as 
% \begin{align}
%     &Q_x = c_x+f_{x}^T V'_{x} \label{eq:ilqg1} \\
%     &Q_u = c_u+f_{u}^T V'_{u} \label{eq:ilqg2} \\
%     &Q_{xx} = c_{xx}+f_{x}^T V'_{xx}f_{x} + V'_x \cdot f_{xx}  \label{eq:ilqg3} \\
%     &Q_{ux} = c_{ux}+f_{u}^T V'_{xx}f_{x}  + V'_x \cdot f_{ux} \label{eq:ilqg4} \\
%     &Q_{uu} = c_{uu}+f_{u}^T V'_{xx}f_{u}  + V'_x \cdot f_{uu}\label{eq:ilqg5} 
% \end{align}
% where $V' \equiv V_{t+1}$. The final terms in equations \ref{eq:ilqg3}, \ref{eq:ilqg4} and  \ref{eq:ilqg5} are ignored in ILQR. 

% Minimizing equation \ref{eq:ilqg_2nd_order} w.r.t. $\delta u$ gives
% \begin{equation}
%     \delta u^* = arg \min_{\delta u} Q_t(\delta x,\delta u) = -Q_{uu}^{-1}(Q_u+Q_{ux}\delta x)
% \end{equation}
% This gives an open-loop term $k=-Q_{uu}^{-1}Q_u$, along with the feedback gain term $K=-Q_{uu}^{-1}Q_{ux}$. Substituting the policy in equation \ref{eq:ilqg_2nd_order}, we have a quadratic model of the value function:
% \begin{align*}
%     &\Delta V(t) = -\frac{1}{2} Q_u Q_{uu}^{-1}Q_u \\ %\label{eq:ilqg1} \\
%     &V_x(t) = Q_x-Q_u Q_{uu}^{-1}Q_{ux} \\%\label{eq:ilqg2} \\
%     &V_{xx}(t) = Q_xx-Q_{xu} Q_{uu}^{-1}Q_{ux}  %\label{eq:ilqg3}
% \end{align*}

% The backward pass recursively computes the local quadratic models of $V(t)$ and ${k(t), K(t)}$. When the backward pass is completed, a forward pass of the algorithm then computes a new trajectory:
% \begin{align*}
%     &\hat{x}(0)=x(0) \\
%     &\hat{u}_t = u_t+k(t)+K(t)(\hat{x}(t)=x(t))\\
%     &\hat{x}(t+1)=f(\hat{x}(t), \hat{u}_t)
% \end{align*}


We present details of the D2C-ILQR algorithm in the following. The 'forward pass' and `backward pass' algorithms are summarized in Algorithms \ref{model_free_DDP_OL_FP} and \ref{model_free_DDP_OL_BP} respectively. Algorithm \ref{model_free_DDP_feedback} presents the DDP feedback algorithm used to calculate the optimal feedback gain. 

\begin{algorithm}
\footnotesize
 \caption{\strut Forward Pass}
  {\bf Input:} Nominal trajectory - $\mathbb{T}_{nom}^{k}$, previous iteration policy parameters - $\{k_{0:N-1}, K_{0:N-1}\}$ and system and cost parameters - $\mathcal{P}$.\
%   \CommentSty{/* Unpack the previous nominal trajectory.*/}\\
  $\{{\bar{x}_t^{prev}, \bar{u}_t^{prev}}\} \gets \mathbb{T}_{nom}^{k}$.\\
%   \CommentSty{/* Initialize time to 0.*/}\\
  $t \gets 0$.\\
  \While {$t < N$}{
    %\CommentSty{/*$\alpha$ is the line-search parameter.*/} \\
    \CommentSty{/*Simulate one step forward ($\alpha$ is the line-search parameter.)*/}
    \begin{equation*}
    \begin{split}
        {\bar{u}_{t}} &= {\bar{u}_t^{prev}} + \alpha k_t + K_{t} ({\bar{x}_t} - {\bar{x}_t^{prev}}),\\
        {\bar{x}_{t+1}} &= simulate\_forward\_step({\bar{x}_t}, {\bar{u}_t}).
        \end{split}
    \end{equation*}
    $t \leftarrow t + 1$. 
    }
  $\mathbb{T}_{nom}^{k+1}$ $\gets$ $\{{\bf \bar{x}_{0:N}}, {\bf \bar{u}_{0:N-1}}\}.$\\
  \If{$\mathbb{T}_{nom}^{k+1}$ to $\mathbb{T}_{nom}^{k}$ \textnormal{is acceptable}}{
    {\bf return} $\mathbb{T}_{nom}^{k+1}$, true.
  }
  \Else{
    {\bf return} $\mathbb{T}_{nom}^{k}$, false.
  }
  \label{model_free_DDP_OL_FP}
\end{algorithm}
%
\begin{algorithm} 
\footnotesize
  \caption{\strut Backward Pass}
  {\bf Input:} Nominal trajectory - $\mathbb{T}_{nom}^{k}$, previous iteration policy parameters - $\{k_{0:N-1}, K_{0:N-1}\}$, horizon - N and system and cost parameters - $\mathcal{P}$.\\
  \CommentSty{/* Backward pass starts from the final time-step i.e, N-1.*/}\\
  $t \gets N - 1$.\ \\
  Compute $J_{x_N}$ and $J_{x_N x_N}$ using boundary conditions.\\
  \CommentSty{/*Keep a copy of previous policy gains.*/}\\
  $k\_old \gets k_{0:N}$ {and}  $K\_old \gets K_{0:N}$.\\
  
  \While {$t >= 0$}{
  \CommentSty{/*Obtain the Jacobians from simulator rollouts as shown in Section \ref{sys_id_solve}:*/}\\
  $f_{x_t}, f_{u_t} \gets model\_free\_jacobian({ \bar{x}_t},{\bar{u}_t}).$\\
  \CommentSty{/*Obtain the partials of the Q function as follows:*/}
    \begin{equation*}
    \begin{split}
    Q_{x_t} &= c_{x_t}  + h_{x_t}^T J_{x_{t+1}}^{\prime},\\
    Q_{u_t} &= c_{u_t} + h_{u_t}^T J_{x_{t+1}}^{\prime},\\
    Q_{x_t x_t} &= c_{x_t x_t} + h_{x_t}^T J_{x_{t+1} x_{t+1}}^{\prime} h_{x_t}, \\
    Q_{u_t x_t} &= c_{u_t x_t} + h_{u_t}^T (J_{x_{t+1} x_{t+1}}^{\prime} + \mu I_{n_x \times n_x}) h_{x_t}, \\
    Q_{u_t u_t} &= c_{u_t u_t} + h_{u_t}^T (J_{x_{t+1} x_{t+1}}^{\prime} + \mu I_{n_x \times n_x}) h_{u_t}.\\
    \end{split}
\end{equation*}
  \If{$Q_{u_t u_t}$ {\textnormal{is positive-definite}}}{
    \begin{equation*}
    \begin{split}
        k_t &= -Q_{u_t u_t}^{-1} Q_{u_t},\\
        K_t &= -Q_{u_t u_t}^{-1} Q_{u_t x_t}.
        \end{split}
    \end{equation*}
    }
    
%   \Endif
  \Else{
    \CommentSty{/*If $Q_{u_t u_t}$ is not positive-definite, then, abort the backward pass.*/}\\
    {\bf return } $\{ k\_old, K\_old\}$, false.
  }
  \CommentSty{/*Obtain the partials of the value function $J_t$ as follows:*/}
  \begin{equation*}
      \begin{split}
          J_{x_t} &= Q_{x_t} + K_{t}^T Q_{u_t u_t} k_t + K_t^T Q_{u_t} + Q_{u_t x_t}^T k_t,\\
          J_{x_t x_t} &= Q_{x_t x_t} + K_t^T Q_{u_t u_t} K_t + K_t^T Q_{u_t x_t} + Q_{u_t x_t}^T K_t.
      \end{split}
  \end{equation*}
  $t \leftarrow t - 1$ 
  }
  $k\_new = k_{0:N-1},$\\
  $K\_new = K_{0:N-1}.$\\
  {\bf return} $\{k\_new, K\_new\}$, true.
  \label{model_free_DDP_OL_BP}
\end{algorithm}

\begin{algorithm} 
\footnotesize
  \caption{\strut DDP Feedback}
  {\bf Input:} Nominal trajectory - $\mathbb{T}_{nom}^{k}$, horizon - N and system and cost parameters - $\mathcal{P}$.\\
  \CommentSty{/* Start from the final time-step i.e, N-1.*/}\\
  $t \gets N - 1$.\ \\
  Compute $J_{x_N}$ and $J_{x_N x_N}$ using boundary conditions.\\

  \While {$t >= 0$}{
  \CommentSty{/*Obtain the Jacobians from simulator rollouts as shown in Section \ref{sys_id_solve}:*/}\\
  $h_{x_t}, h_{u_t} \gets model\_free\_jacobian({ \bar{x}_t},{\bar{u}_t}).$\\
  \CommentSty{/*Obtain the Hessians from simulator rollouts as shown above:*/}\\
  $h_{x_tx_t}, h_{u_tx_t}, h_{u_tu_t} \gets model\_free\_hessian({ \bar{x}_t},{\bar{u}_t}).$\\
  \CommentSty{/*Obtain the partials of the Q function as follows:*/}
    \begin{equation*}
    \begin{split}
    Q_{x_t} &= c_{x_t}  + h_{x_t}^T J_{x_{t+1}}^{\prime},\\
    Q_{u_t} &= c_{u_t} + h_{u_t}^T J_{x_{t+1}}^{\prime},\\
    Q_{x_t x_t} &= c_{x_t x_t} + h_{x_t}^T J_{x_{t+1} x_{t+1}}^{\prime} h_{x_t} + J_{x_{t+1}}^{\prime}h_{x_tx_t}, \\
    Q_{u_t x_t} &= c_{u_t x_t} + h_{u_t}^T (J_{x_{t+1} x_{t+1}}^{\prime} + \mu I_{n_x \times n_x}) h_{x_t} + J_{x_{t+1}}^{\prime}h_{u_tx_t}, \\
    Q_{u_t u_t} &= c_{u_t u_t} + h_{u_t}^T (J_{x_{t+1} x_{t+1}}^{\prime} + \mu I_{n_x \times n_x}) h_{u_t} + J_{x_{t+1}}^{\prime}h_{u_tu_t}.\\
    \end{split}
\end{equation*}
  \If{$Q_{u_t u_t}$ {\textnormal{is positive-definite}}}{
    \begin{equation*}
    \begin{split}
        k_t &= -Q_{u_t u_t}^{-1} Q_{u_t},\\
        K_t &= -Q_{u_t u_t}^{-1} Q_{u_t x_t}.
        \end{split}
    \end{equation*}
    }
    
%   \Endif
  \Else{
    \CommentSty{/*If $Q_{u_t u_t}$ is not positive-definite, then, abort the backward pass.*/}\\
    {\bf return } error.
  }
  \CommentSty{/*Obtain the partials of the value function $J_t$ as follows:*/}
  \begin{equation*}
      \begin{split}
          J_{x_t} &= Q_{x_t} + K_{t}^T Q_{u_t u_t} k_t + K_t^T Q_{u_t} + Q_{u_t x_t}^T k_t,\\
          J_{x_t x_t} &= Q_{x_t x_t} + K_t^T Q_{u_t u_t} K_t + K_t^T Q_{u_t x_t} + Q_{u_t x_t}^T K_t.
      \end{split}
  \end{equation*}
  $t \leftarrow t - 1$ 
  }
  $K = K_{0:N-1}.$\\
  {\bf return} $\{K\}$, true.
  \label{model_free_DDP_feedback}
\end{algorithm}

% \subsection*{Estimation of Jacobians: Linear Least Squares by Central Difference (LLS-CD)}
% \label{sys_id_solve_supplementary}

% \textit{Note: The following is a more detailed discussion of section 4.1.1 in the main paper.}
% % We make a preliminary analysis on the number of evaluations required in the above algorithm. If the horizon is `$h$' and the number of iterations required to converge are `$n$', the algorithm requires us to estimate each of the $f_{\bf x_t}$ and $f_{\bf u_t}$ `$nh$' times. 


% % \begin{equation*}
% % \begin{split}
% %     &f({\bf \bar{x}_t} + \delta {\bf x_t}, {\bf \bar{u}_t} + \delta {\bf u_t}) = f({\bf \bar{x}_t}, {\bf \bar{u}_t}) + \begin{bmatrix} f_{\bf x_t}  f_{\bf u_t} \end{bmatrix} \begin{bmatrix}  \delta {\bf x_t} \\ \delta {\bf u_t} \end{bmatrix} + \\&\frac{1}{2} \begin{bmatrix} \delta {\bf x_t}^T  \delta {\bf u_t}^T \end{bmatrix} \begin{bmatrix} f_{\bf x_t x_t}  f_{\bf x_t u_t}\\ f_{\bf u_t x_t}  f_{\bf u_t u_t}\end{bmatrix} \begin{bmatrix} \delta {\bf x_t} \\ \delta {\bf u_t}\end{bmatrix} +
% %     O(\| \delta {\bf x_t}\|^3 + \| \delta {\bf u_t}\|^3)\\
% %     &f({\bf \bar{x}_t} - \delta {\bf x_t}, {\bf \bar{u}_t} - \delta {\bf u_t}) = f({\bf \bar{x}_t}, {\bf \bar{u}_t}) - \begin{bmatrix} f_{\bf x_t} f_{\bf u_t} \end{bmatrix} \begin{bmatrix}  \delta {\bf x_t} \\ \delta {\bf u_t} \end{bmatrix} + \\&\frac{1}{2} \begin{bmatrix} \delta {\bf x_t}^T \delta {\bf u_t}^T \end{bmatrix} \begin{bmatrix} f_{\bf x_t x_t}  f_{\bf x_t u_t}\\ f_{\bf u_t x_t}  f_{\bf u_t u_t}\end{bmatrix} \begin{bmatrix} \delta {\bf x_t} \\ \delta {\bf u_t}\end{bmatrix}+
% %     O(\| \delta {\bf x_t}\|^3 + \| \delta {\bf u_t}\|^3)\\
% %   \end{split}
% % \end{equation*}
% Using Taylor's expansions of `$h$' (for generality, $h$ is the non-linear model of Section 2) about the nominal trajectory $(\bar{x}_t,  \bar{u}_t)$ on both the positive and the negative sides, we obtain the following central difference equation:\\
% $
%     h(\bar{x}_t + \delta x_t, \bar{u}_t + \delta u_t) - h(\bar{x}_t - \delta x_t, \bar{u}_t - \delta  u_t) =~2 \begin{bmatrix} h_{x_t} & h_{u_t} \end{bmatrix} \begin{bmatrix}  \delta {x_t} \\ \delta {u_t} \end{bmatrix} + O(\| \delta {x_t}\|^2 + \| \delta {u_t}\|^2).
% $
% Multiplying by $\begin{bmatrix} \delta {x_t}^T & \delta {u_t}^T \end{bmatrix}$ on both sides to the above equation:
% \begin{equation*}
%     \begin{split}
%     \begin{bmatrix}h({\bar{x}_t} + \delta {x_t}, {\bar{u}_t} + \delta {u_t}) -  h({\bar{x}_t} - \delta {x_t}, {\bar{u}_t} - \delta {u_t})\end{bmatrix} 
%      \times \begin{bmatrix} \delta {x_t}^T & \delta {u_t}^T \end{bmatrix} 
%     % &= 2 \begin{bmatrix} f_{\bf x_t} & f_{\bf u_t} \end{bmatrix} \begin{bmatrix}  \delta {\bf x_t} \\ \delta {\bf u_t} \end{bmatrix} \begin{bmatrix} \delta {\bf x_t}^T & \delta {\bf u_t}^T \end{bmatrix}+ O(\| \delta {\bf x_t}\|^4 + \| \delta {\bf u_t}\|^4)\\
%      =2 \begin{bmatrix} h_{x_t} & h_{u_t} \end{bmatrix} \begin{bmatrix}  \delta {x_t} \delta {x_t}^T & \delta {x_t} \delta {u_t}^T \\ \delta {u_t} \delta {x_t}^T  & \delta {u_t} \delta {u_t}^T \end{bmatrix} \nonumber \\~~~~~~~~~~~~
%      + O(\| \delta {x_t}\|^3 + \| \delta {u_t}\|^3)
%      \end{split}
% \end{equation*}
% Assuming that $\begin{bmatrix}  \delta {x_t} \delta {x_t}^T & \delta {x_t} \delta {u_t}^T \\ \delta {u_t} \delta {x_t}^T  & \delta {u_t} \delta {u_t}^T \end{bmatrix}$ is invertible (which will later be proved to be true by some assumptions), let us perform inversions on either sides of the above equation as follows:
% % \begin{equation*}
% %     \begin{split}
% %     &\begin{bmatrix}f({\bf \bar{x}_t} + \delta {\bf x_t}, {\bf \bar{u}_t} + \delta {\bf u_t}) - f({\bf \bar{x}_t} - \delta {\bf x_t}, {\bf \bar{u}_t} - \delta {\bf u_t})\end{bmatrix} \times\\
% %     &\begin{bmatrix} \delta {\bf x_t}^T & \delta {\bf u_t}^T \end{bmatrix} \begin{bmatrix}  \delta {\bf x_t} \delta {\bf x_t}^T & \delta {\bf x_t} \delta {\bf u_t}^T \\ \delta {\bf u_t} \delta {\bf x_t}^T  & \delta {\bf u_t} \delta {\bf u_t}^T \end{bmatrix}^{-1} = \\&2 \begin{bmatrix} f_{\bf x_t} & f_{\bf u_t} \end{bmatrix} +
% %      O(\| \delta {\bf x_t}\|^2 + \| \delta {\bf u_t}\|^2)
% %      \end{split}
% % \end{equation*}
% % $\implies$ 
% \begin{equation}
%     \begin{split}
%     \begin{bmatrix} h_{x_t}~h_{u_t} \end{bmatrix} 
%     &=\frac{1}{2}\begin{bmatrix} h({\bar{x}_t} + \delta {x_t}, {\bar{u}_t} + \delta {u_t}) - h({\bar{x}_t} - \delta {x_t}, {\bar{u}_t} - \delta {u_t})\end{bmatrix}  \times\begin{bmatrix} \delta {x_t}^T & \delta {u_t}^T \end{bmatrix} \begin{bmatrix}  \delta {x_t} \delta {x_t}^T~ \delta {x_t} \delta {u_t}^T \\ \delta {u_t} \delta {x_t}^T ~\delta {u_t} \delta {u_t}^T \end{bmatrix}^{-1}\\ &~~~~~~~~~~~~~~~~~~+ O(\| \delta {x_t}\| + \| \delta {u_t}\|)
%      \label{eq : model_free_DDP_jacobian_raw1}
%      \end{split}
% \end{equation}
% Equation \eqref{eq : model_free_DDP_jacobian_raw1} solves for Jacobians, $h_{x_t}$ and $h_{u_t}$, simultaneously. It is noted that the above formulation requires only 2 evaluations of $h(.)$, given the nominal state and control $\-$ (${\bar{x}_t},{\bar{u}_t}$). The remaining terms (also, the error in the evaluation) are of the order that is linear in $\delta {x_t}$ and $\delta {u_t}$. The following extends equation \eqref{eq : model_free_DDP_jacobian_raw1} to be used in practical implementations (sampling).\\
% We are free to choose the distribution of $\delta {x_t}$ and $\delta {u_t}$. We assume both are i.i.d. Gaussian distributed random variables with zero mean and a standard deviation of $\sigma$.~This ensures that $\begin{bmatrix}  \delta {x_t} \delta {x_t}^T & \delta {x_t} \delta {u_t}^T \\ \delta {u_t} \delta {x_t}^T  & \delta {u_t} \delta {u_t}^T \end{bmatrix}$ is invertible. Let `$n_s$' be the number of samples for each of the random variables, $\delta {x_t}$ and $\delta {u_t}$. Denote the random samples as $\delta {X_t} = \begin{bmatrix} \delta {x_t^1}& \delta {x_t^2}& \ldots &\delta {x_t^{n_s}}\end{bmatrix}$, $\delta {U_t} = \begin{bmatrix} \delta {u_t^1} &\delta {u_t^2}& \ldots& \delta {u_t^{n_s}}\end{bmatrix}$ and $\delta Y_t = \begin{bmatrix} \delta X_t & \delta U_t \end{bmatrix}$. Then $\begin{bmatrix} h_{x_t} & h_{u_t} \end{bmatrix}$ is given by the following (via standard least squares):
% \begin{equation}
%     \begin{split}
%     &\begin{bmatrix} h_{x_t}~h_{u_t} \end{bmatrix} = H \delta Y_t^T (\delta Y_t\delta Y_t^T)^{-1} \\
%     &H = \begin{bmatrix} h({\bar{x}_t} + \delta {x_t^1}, {\bar{u}_t} + \delta {u_t^1}) - h({ \bar{x}_t} - \delta {x_t^1}, {\bar{u}_t} - \delta {u_t^1})\\ h({\bar{x}_t} + \delta {x_t^2}, {\bar{u}_t} + \delta {u_t^2}) - h({\bar{x}_t} - \delta {x_t^2}, {\bar{u}_t} - \delta {u_t^2}) \\ \vdots  \\h({\bar{x}_t} + \delta {x_t^{n_s}}, {\bar{u}_t} + \delta {u_t^{n_s}}) - h({\bar{x}_t} - \delta {x_t^{n_s}}, {\bar{u}_t} - \delta {u_t^{n_s}})\end{bmatrix}
%      \label{eq : model_free_DDP_jacobian1}
%      \end{split}
% \end{equation}
% Let us consider the terms in the matrix $\delta Y_t \delta Y_t^T=\begin{bmatrix}  \delta {X_t} \delta {X_t}^T & \delta {X_t} \delta {U_t}^T \\ \delta {U_t} \delta {X_t}^T  & \delta {U_t} \delta {U_t}^T \end{bmatrix}$.~$\delta {X_t} \delta {X_t}^T = \sum_{i=1}^{n_s} \delta {x_t}^i {\delta {x_t}^i}^T$. Similarly, $\delta {U_t} \delta {U_t}^T = \sum_{i=1}^{n_s} \delta {u_t}^i {\delta {u_t}^i}^T$, $\delta {U_t} \delta {X_t}^T = \sum_{i=1}^{n_s} \delta {u_t}^i {\delta {x_t}^i}^T$ and $\delta {X_t} \delta {U_t}^T = \sum_{i=1}^{n_s} \delta {x_t}^i {\delta {u_t}^i}^T$. From the definition of sample variance, for a large enough $n_s$, we can write the above matrix as 
% \begin{equation*}
% \begin{split}
%     \delta Y_t \delta Y_t^T &= \begin{bmatrix} \sum_{i=1}^{n_s} \delta {x_t}^i {\delta {x_t}^i}^T & \sum_{i=1}^{n_s} \delta {x_t}^i {\delta {u_t}^i}^T \\ \sum_{i=1}^{n_s} \delta {u_t}^i {\delta {x_t}^i}^T & \sum_{i=1}^{n_s} \delta {u_t}^i {\delta {u_t}^i}^T
%     \end{bmatrix}\\ &\approx \begin{bmatrix} \sigma^2(n_s - 1) {\text I_{n_x}} & {\text 0_{n_x \times n_u}} \\ 0_{n_u \times n_x} & \sigma^2 (n_s - 1) {\text I_{n_u}}\end{bmatrix} \\
%     &= \sigma^2 (n_s - 1){\text I}_{(n_x+n_u) \times (n_x+n_u)}
% \end{split}
% \end{equation*}

% \textit{Sample Complexity.} 
% Given that we have high enough number of samples $n_s$, typically `$O(n_x + n_u)$', the above approximation holds good. The reason is as follows. Note that the above least squares procedure converges when the matrix $\delta Y_t \delta Y_t^T$ converges to the identity matrix. This is entirely equivalent to estimation of the covariance of the  random vector $[\delta x_t \ \delta u_t]$ where $\delta x_t$, and $\delta u_t$ are Gaussian i.i.d. samples. Thus, it follows that the number of samples is $O(n_x+n_u)$, given $n_x+n_u$ is large enough \cite{HDP-book}. \\
% Note that if one were to use an FD procedure, the number of samples would be $O(n_x(n_x+n_u)) >> O(n_x+n_u)$. In fact, this behaviour is clearly apparent in our empirical results where FD is more efficient for low dimensional examples, while the LLS-CD procedure rapidly becomes much more efficient as the size of the examples increases. This has very important ramifications since the overwhelming bulk of the computations in our D2C implementation is in the estimation of these system dynamics. 

% \subsection*{Guarantees for ILQR}
% %\textcolor{red}{Can you add the iLQR/ DDP insight here?}\\
% As has been mentioned previously, iLQR is much more efficient than the related DDP procedure \cite{ddp} which requires the availability of the second order dynamics terms. Albeit this is known empirically \cite{ilqg2}, it is not clear as to why iLQR should provide a solution of the same quality as DDP? \\
% The reasoning for this as follows. 
% The DDP procedure is simply a sequential quadratic programming (SQP) procedure for the trajectory optimization problem, where the dynamics are the constraints in the optimization problem. In SQP, the Lagrangian, i.e., the cost function augmented with the constraints using the Lagrange multipliers, $\mathcal{L}(x,\lambda) = c(x) + \lambda h(x)$, where $c(x)$ is the cost function and $h(x) =0$ are the constraints, is expanded to second order about the current solution. In the context of trajectory optimization, this amounts to expanding the cost function to second order which also results in second order expansion of the dynamics. The only difference between DDP and iLQR is that, in iLQR, the second order expansion of the dynamics is neglected in the optimization problem.
% This is similar to idea of neglecting second order terms in Gauss-Newton's method (identical to iLQR) as compared to Newton's method (identical to DDP).
% Moreover, the guarantees for SQP, i.e., convergence to a stationary point of the augmented cost function still holds for iLQR. Therefore, it follows that we can expect iLQR to converge to a stationary point of the optimal control problem.\\
% Next, note that due to the Method of Characteristics development in the previous section, if the dynamics are affine in control and the cost is quadratic in control, it follows that satisfying the necessary conditions for optimality, which iLQR is guaranteed to do under mild conditions, one is assured of the global minimum to the problem. Then, a perturbation expansion of the characteristic equations about this optimal is guaranteed to give us at least a local solution to the HJB equation.% due to Proposition~\ref{T-PFC}.
% %Since the inversion of an identity matrix is trivial and always exists, the above matrix is invertible in equation \eqref{eq : model_free_DDP_jacobian1}. Thus, one can calculate $f_{\bf x}$ and $f_{\bf u}$ this way during the backward pass. For the sake of convenience in the later sections, let us refer to this method as `Linear Least Squares by Central Difference (LLS-CD)'. 
% %The entire algorithm to determine the optimal nominal trajectory in a model-free fashion is summarized together in Algorithm \ref{model_free_DDP_OL}. The detailed forward and backward pass functions are shown in Algorithm \ref{model_free_DDP_OL_FP} and \ref{model_free_DDP_OL_BP} respectively in the supplementary material.

\subsection*{DDP Feedback Gain Calculation}
Once the optimal nominal trajectory is obtained with ILQR, one DDP back pass is conducted to find the linear optimal feedback gain as shown in Algorithm \ref{model_free_DDP_feedback}. Then the linear feedback is wrapped around the nominal control sequence ($u_t = \bar{u}_t + K_t\delta x_t$),where $\delta x_t$ is the state deviation from the nominal state $\bar{x}_t$.

% \sr
% \begin{align}
% z_i &= \begin{bmatrix} \delta {x}^T & \delta {u}^T \end{bmatrix} \begin{bmatrix} h_{xx}^{(i)}  & h_{xu}^{(i)}  \\ h_{ux}^{(i)}  & h_{uu}^{(i)}  \end{bmatrix} \begin{bmatrix}  \delta {x} \\ \delta {u} \end{bmatrix} \nonumber \\  \nonumber
% &= \sum_{j=1}^{n_s} \sum_{k=1}^{n_s} \dfrac{\partial^2 h_i}{\partial x_j \partial x_k} \delta x_j \delta x_k + 2 \sum_{p=1}^{n_u} \sum_{q=1}^{n_s} \dfrac{\partial^2 h_i}{\partial u_p \partial x_q} \delta u_p \delta x_q + \sum_{d=1}^{n_u} \sum_{h=1}^{n_u} \dfrac{\partial^2 h_i}{\partial u_d \partial u_h} \delta u_d \delta u_h \\ \nonumber
% &= \underbrace{\begin{bmatrix} \delta {x_1}^2 & \delta {x_1} \delta {x_2} & \cdots & \delta {x_1} \delta {u_{n_u}} & \delta {x_2}^2 & \delta {x_2} \delta {x_3} & \cdots& \delta {u^2_{n_u}}\end{bmatrix}}_{\delta {XU}}  \underbrace{\begin{bmatrix} \dfrac{\partial^2 h_i}{\partial x_1^2} \\ \\ 2 \dfrac{\partial^2 h_i}{\partial x_1 \partial x_2} \\ \vdots \\ 2 \dfrac{\partial^2 h_i}{\partial x_1 \partial u_{n_u}} \\ \\ \dfrac{\partial^2 h_i}{\partial x_2^2} \\ \\ 2 \dfrac{\partial^2 h_i}{\partial x_2 \partial x_3} \\ \vdots \\ \dfrac{\partial^2 h_i}{\partial {u^2_{n_u}}}\end{bmatrix}}_{H_i},\\
% \end{align}
% % \begin{bmatrix} \delta {x_1} & \delta {x_2} & \cdots & \delta {x_{n_s}} & \delta {u_1} & \delta {u_2} & \cdots & \delta {u_{n_u}} \end{bmatrix} 

% where $h_{xx}^{(i)} = \left.\dfrac{\partial^2 h_i}{\partial x^2}\right|_{x=t}$, $z_i$ is the $i^{th}$ element of vector $z_t$ and $h_i$ is the $i^{th}$ element of the dynamics vector $h(x_t, u_t)$. Multiplying on both sides by $\delta XU^T$ and apply standard Least Square method:
% $H_i = (\delta XU^T \delta XU)^{-1} \delta XU^T Z_i$. Then repeat for $i=1,2,...,n_s$ to get the estimation for the Hessian tensor.

==> MaterialControl.tex <==
\subsection{Model Based Control for Microstructure Dynamics}\label{append:control}
 
%\subsection{Controller for Decoupled Dynamics Model}
In this section, we derive a simple control scheme to control the inputs to each grid point in the material, so as to reach the desired phase distribution. Suppose we discretize the material domain, and let, for a point at location $(x_i,y_j)$, the instantaneous order parameter be $\phi_{ij}(t)$, while $\phi_{ij}^F$ defines the final desired state for that point.

The Allen-Cahn equation has an interesting structure, suppose we neglect the diffusion term, i.e., set $\gamma =0$ in \eqref{eq:Dyn_main}. Also, assume that the control input is time-invariant at any grid point $(i,j)$, i.e., $(T(t),h(t))= (\bar{T}_{ij},\bar{h}_{ij})$ for all time $t$. Thus, setting $\gamma=0$, Equation \ref{eq:Dyn_main} is reduced to the ordinary differential equation:

\begin{align}
    &\frac{d \phi_{ij}}{dt}= -M(4\phi_{ij}^3+2\phi_{ij} \bar{T}_{ij}+\bar{h}_{ij}),
\end{align}
where we note that the phase field at the different points $(i,j)$, in the domain now evolve completely independent of the others. 
At steady-state, $\phi_{ij}=\phi_{ij}^F$. Thus, for the time-invariant control inputs, we get the constraint:
\begin{align}
    &4(\phi_{ij}^F)^3+2\phi_{ij}^F \bar{T}_{ij}+\bar{h}_{ij} = 0. \label{eq:constraint}
\end{align}

Since the constraint above can be satisfied by a family of control inputs $u_{ij} = (\bar{T}_{ij},\bar{h}_{ij})$, in order to regularize the problem, a cost function $(J)$ is defined, and the control input $u_{ij} = (\bar{T}_{ij},\bar{h}_{ij})$ which minimizes the cost is chosen. 
\begin{align}
    &J(\phi_{ij}, u_{ij})=\frac{1}{2}\phi_{ij}^T Q\phi_{ij}+\frac{1}{2}u_{ij}^T R u_{ij}
\end{align}
where $Q$ and $R$ are some positive definite matrices. The Hamiltonian for this problem can be written as
\begin{align}
    &H = \frac{1}{2}\phi_{ij}^{T} Q\phi_{ij}+\frac{1}{2}u_{ij}^T R u_{ij} + \lambda^T (4(\phi_{ij}^F)^3+2\phi_{ij}^F \bar{T}_{ij}+\bar{h}_{ij})
\end{align}
We apply the necessary conditions for constrained optimization to obtain:
\begin{align*}
    &\dot{\lambda} = -\frac{\partial H}{\partial \phi}=-Q\phi_{ij}^F-\lambda(2\bar{T}_{ij}+12(\phi_{ij}^F)^2),\\
    &\frac{\partial H}{\partial T_{ij}}=\bar{T}_{ij}+2\lambda\phi_{ij}^F=0,\\
    &\frac{\partial H}{\partial h_{ij}}=\bar{h}_{ij}+\lambda =0
\end{align*}
We finally substitute these values back into the constraint (Eq. \ref{eq:constraint}) to get the desired time invariant control input as 
\begin{align}
    \bar{T}_{ij}=\frac{-8(\phi_{ij}^F)^4}{1+4(\phi_{ij}^F)^2},  \bar{h}_{ij}=\frac{-4(\phi_{ij}^F)^3}{1+4(\phi_{ij}^F)^2}
\end{align}

The values of the control above assure us that the phase variable converges to the desired steady state value, in the absence of the diffusion. However, we note that the phase can still get stuck in a local minimum that is different from the desired value, if the initial condition is not close enough to the desired steady state value. We use this physics based control scheme as a baseline for comparison with a data based optimal controller, which considers the full Allen Cahn dynamics, that we propose in the next Section.


==> Replanning.tex <==
\subsubsection{Model Predictive Control}

To reduce the variance of the policy in high noise regimes, we advocate the use of a rapid open loop solver along with replanning at every step, i.e. a \textbf{Model-Predictive Control} approach, to solve the RL problem, since MPC should be able to recover the global optimality for these problems \cite{mohamed2020near}.

 The recursive MPC algorithm implemented, which uses a fast and reliable local-planner, is summarised in Algorithm \ref{alg3}, and Figure \ref{fig:replan_error} compares the robustness to noise between the stochastic policy obtained from the recursive MPC with the decoupled closed-loop feedback policy at varying noise regimes.
 
 \begin{algorithm}
    \caption{Recursive MPC Algorithm}
    \label{alg3}
   {\bf 1)}  \textit{Given:} Initial state $x_0$, time horizon $T$, cost $c(x,u)=l(x)+\frac{1}{2}ru^2$, and terminal cost $c_T(x)$.\\
  {\bf 2)} Set $H=T$, $x_i = x_0$.\\
%   {\bf 3)} Solve the Riccati equations for each step along the nominal trajectory for feedback gain $\{ K_t \}_{t = 0}^{T-1}$.\\
%   {\bf 4)} Apply the closed-loop control policy,
  
\While{$H >0$}{
  \begin{enumerate}
        \item Solve the open-loop(deterministic) optimal control problem for initial state $x_i$ and horizon $H$. Let the optimal sequence be $U^*=\{u_0, u_1,...u_{H-1}\}$.
        \item Apply the first control $u_0$ to the stochastic system,\\
        and observe the next state $x_n$.
        \item Set $H=H-1, x_i = x_n$
\end{enumerate}
}
\end{algorithm}

 We observe that re-planning at every time-step easily recovers the optimality over all noise-regimes. Also, owing to the rapid convergence of the open-loop solvers for the material micro-structures, the extra computation cost which arises due to the repeated iterations of the open-loop solver, is not very significant, and can be reduced even further by integrating the MPC approach with a warm-start optimization (Figure \ref{fig:rep_train_times}).
 


\begin{figure}[!htb]
%\captionsetup{width=1\linewidth}



\begin{multicols}{2}
    %\hspace{3.2cm}
      \subfloat[]{\includegraphics[width=1\linewidth]{images/Replan_comp_plots/comp_time_replan.png}}    
      \subfloat[]{\includegraphics[width=\linewidth]{images/Replan_comp_plots/cml_comp_time_replan.png}}
      %\subfloat[t=1.25s]{\includegraphics[width=0.8\linewidth]{images/50per/file49.png}}\\ 
\end{multicols}
%\begin{multicols}{6}
%\captionsetup{width=.75\textwidth}
    \caption{{Computation times for re-planning with the recursive MPC approach}} 
%\end{multicols}

\label{fig:rep_train_times}
\end{figure}

==> Reviews_CDC2020.tex <==
% Reviewer 2 of CDC 2020 submission 1279

% Comments to the author
% ======================

% In the submission „Optimal Control of Material
% Micro-Structures” the authors consider a so called
% Allen-Cahn equation, which is an diffusion equation for the
% mixture of two phases, driven by nonlinear indomain
% actuation. For 100% concentration of one phase, the state
% is equal -1, for 100 % concentration of the other phase,
% the state is equal +1. For the actuation both the
% temperature and an external force field can be assigned
% arbitrarily for any time and location. A “model based
% control” (which is only the steady-state control input) is
% compared with the proposed “decoupled data based control
% (D2C)”. The latter, is based on an optimization of an
% feedforward trajectory and an feedback. 

% I cannot recommend acceptance, for the following reasons:
% The distributed character of the plant is not considered.
% For the “model based control”, the diffusion is ignored and
% only a constant control input is considered. For the “D2C”
% approach, the dynamics are approximated with a lumped,
% time-discrete system that results from an identification
% and is not deduced by the distributed system model. In
% general, the aspect, that the state is bounded on [-1, +1],
% is ignored in the design. 


% Reviewer 3 of CDC 2020 submission 1279

% Comments to the author
% ======================

% The paper addresses an optimal control problem for material
% micro-structures. The paper is rather unusual for classical
% control theory, since strongly relying on physical
% consideration of so-called Phase Fields and associated
% material properties. Still the paper might be interesting
% for CDC auditorium if properly written. Several remarks and
% comments are given below.

% -	“for the control of these systems” might be
% confusing, since not fully clear whether production or
% exploitation processes of material micro-structures are
% meant here. The Authors are welcome to put more
% straightforward description of problem statement within the
% Introduction part.

% -	“Number of new algorithms” you are referring to,
% i.e. [14]-[16] are all arXiv records. Please elaborate more
% on presenting state of the art and including also adequate
% available published literature.

% -	Better distinguish your recent contribution from
% the previous work [18].


% -	By your assumption of \phi, after eq. (1), it has
% only two binary states. This provides the system with a
% kind of hybrid, correspondingly switching dynamics. How do
% you deal with this, correspondingly capture the transitions
% between such two-state (phases) of the system?


% -	In view of that T is one of your control variables,
% temperature, an exposition in Sec. I.A-B with discrete
% values, like T={-2,-1,0,1,2} is less clear, or at  least
% not clear from reading.

% -	In Section IV, the step from the nonlinear affine
% in control dynamics (10) to the linearized state-space
% notation is not well described. In total, the Section IV,
% which is more relevant from the control viewpoint, is not
% fluently readable.

% -	In total, the Algorithm 1 appears as an iterative
% procedure of state discretization, obtaining set of local
% LTV models, and designing standard LQR regulator by Riccati
% approach. What is here special or new as for control
% design?

% -	The analysis of resulted control system dynamics
% and stability related issues are missing. 

% -	The overall presentation of the Section V can be
% improved, for making evaluation, correspondingly, test
% scenarios more comprehensible for readers.



% Reviewer 4 of CDC 2020 submission 1279

% Comments to the author
% ======================

% Content
% The authors apply the decoupled data based control approach
% to control the distributed parameter system describing
% material micro-structures. The multi-phase microstructure
% is described the Allen-Cahn equation. The control, is
% basically the offline computed feed-forward control which
% is constant over time.

% The paper is well written and deals with an interesting
% topic. 

% Major remarks:

% The authors should comment more detailed on the possibility
% of reaching only local minima. 

% %% COVERED IN AISTATS PAPER

% Why are the input restricted to be constant? 

% The linear time-varying system identification section
% should be detailed further. A comparison to other
% techniques would be interesting.

% Minor remarks:
% It would be interesting to know, which kind of application
% the authors have in mind, as it is difficult to generate
% two inputs over a plane, e.g. only a temperature
% distribution might be achieves with local heating elements.

% The results of the baseline controller in comparison to the
% optimized control results would be interesting.


